On-Chain Analysis of Smart Contract Dependency Risks on Ethereum

In this paper, we present the first large-scale empirical study of smart contract dependencies, analyzing over 41 million contracts and 11 billion interactions on Ethereum up to December 2024. Our results yield four key insights: (1) 59% of contract transactions involve multiple contracts (median of 4 per transaction in 2024) indicating potential smart contract dependency risks; (2) the ecosystem exhibits extreme centralization, with just 11 (0.001%) deployers controlling 20.5 million (50%) of alive contracts, with major risks related to factory contracts and deployer privileges; (3) three most depended-upon contracts are mutable, meaning large parts of the ecosystem rely on contracts that can be altered at any time, which is a significant risk, (4) actual smart contract protocol dependencies are significantly more complex than officially documented, undermining Ethereum's transparency ethos, and creating unnecessary attack surface. Our work provides the first large-scale empirical foundation for understanding smart contract dependency risks, offering crucial insights for developers, users, and security researchers in the blockchain space.

==> tables/2024_call.tex <==

\begin{table*}[ht]
\centering
\begin{tabular}{|r|l|l|l|}
\hline
% \textbf{Callee Address} & 
\textbf{Count} & \textbf{Label} & \textbf{Proxy?} & \textbf{supplier}\\
\hline
% 0xc02aaa39b223fe8d0a0e5c4f27ead9083c756cc2 &
179,418,544 & Wrapped ETH & No & https://sky.money/\\
% 0xdac17f958d2ee523a2206206994597c13d831ec7 & 
64,467,585 & Tether Token & No & https://www.bitfinex.com/\\
% 0x3fc91a3afd70395cd496c647d5a6cc9d4b2b7fad &
44138004 & Uniswap: Universal Router & No & Uniswap \\
% 0xa0b86991c6218b36c1d19d4a2e9eb0ce3606eb48 &  https://www.coinbase.com/blog/usdc-v2-upgrading-a-multi-billion-dollar-erc-20-token& 
35,129,242 & USDC Coin & Yes & Circlehttps://www.usdc.com/\\

% 0x000000000022d473030f116ddee9f6b43ac78ba3 & 
38,838,029 & Uniswap Protocol: Permit2 & No &Uniswap\\

% 0xe37e799d5077682fa0a244d46e5649f71457bd09 &
14992275 & ? & No & 1inch \\

% 0x7a250d5630b4cf539739df2c5dacb4c659f2488d 
13,654,164 & Uniswap V2 Router & No &Uniswap \\
% 0x1111111254EEB25477B68fb85Ed929f73A960582 &
11435759 & Aggregation Router V5 & No & 1inch \\

% 0x22f9dcf4647084d6c31b2765f6910cd85c178c18 &
10758179 & 0x: Exchange Proxy Flash Wallet
0.00 & Yes & https://0x.org/ \\

\hline
\end{tabular}
\caption{2024: Callee Addresses of call}
\label{tab:callee_addresses_call}
\end{table*}

==> tables/2024_delegatecall.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{|r|l|l|l|}
\hline
% \textbf{Callee Address} & 
\textbf{Count} & \textbf{Label} & \textbf{Proxy?} & \textbf{supplier}\\
\hline
% 0x43506849d7c04f9138d1a2050bbf3a0c054402dd & delegatecall &  https://etherauthority.io/usdc-token-smart-contract-audit/
55058897 & - FiatTokenV2\_2 & Yes & Circle(USDC) \\
% 0x4bba9b6b49f3dfa6615f079e9d66b0aa68b04a4d & delegatecall 
- & Math & No & XEN\\
% 0xd9db270c1b5e3bd161e8c8503c55ceabee709552 & delegatecall & 
- & Safe: Singleton 1.3.0 & Yes & Gnosis \\
% 0x2b33cf282f867a7ff693a66e11b0fcc5552e4425 & delegatecall & 
6068411 & Lido: DAO Impl 1.0.0 & Yes & dev.izqui.eth\\ 
% 0x17144556fd3424edc8fc8a4c940b2d04936d17eb
5689505 &Lido: stETH Token Impl 2.0.0 & No & Lido \\
% 0x0a252663dbcc0b073063d6420a40319e438cfa59
5688149 & XEN token & Yes & XEN \\
%  0x46Affe1b4f3fc41581Fd20FbAF055daeAb80A8b5
4837741 & ? & Yes & ? \\
% 0x1B47A665364bC15C28B05f449B53354d0CefF72f
3793753 & Ether.fi & Yes & Etherfi\\
% 0x0de8bf93da2f7eecb3d9169422413a9bef4ef628 & delegatecall & 
3382201 & CoinTool: XEN Batch Minter & Yes & https://ct.app/dashboard\\
% 0xebaed7a81c298b24ee6d59c22698a951dc448e01
3148401 & -L1MessageQueueWithGasPriceOracle & No & Scroll \\


\hline
\end{tabular}
\caption{2024: Summary of Callee Addresses(delegeatecall) and Associated Counts}
\label{tab:callee_addresses_delegatecall}
\end{table*}

==> tables/2024_most_called_based_on_call_number.tex <==

\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|}
    \hline
        to\_address & caller\_count & call\_count \\ \hline
        % 0xc02aaa39b223fe8d0a0e5c4f27ead9083c756cc2 
        WETH & 1089769 & 347585215 \\ \hline
        % 0x0000000000000000000000000000000000000002 
        0x02 & 42092 & 86980243 \\ \hline
        % 0xdac17f958d2ee523a2206206994597c13d831ec7 
        
        USDT & 8308677 & 82806179 \\ \hline
        % 0xa0b86991c6218b36c1d19d4a2e9eb0ce3606eb48
        USDC & 3409866 & 54947812 \\ \hline
        % 0x43506849d7c04f9138d1a2050bbf3a0c054402dd 
        
        FiatTokenV2\_2(USDC Impl) & 21 & 54083480 \\ \hline
        % 0x0000000000000000000000000000000000000001
        0x01 & 157208 & 46851096 \\ \hline
        % 0x3fc91a3afd70395cd496c647d5a6cc9d4b2b7fad 
        Uniswap: Universal Router& 2318539 & 42000820 \\ \hline
        % 0x4bba9b6b49f3dfa6615f079e9d66b0aa68b04a4d 
        Math(Xen crypto)& 1 & 27471992 \\ \hline
        % 0x0000000000000000000000000000000000000004 
        0x04 & 24938 & 24324839 \\ \hline
        % 0x000000000022d473030f116ddee9f6b43ac78ba3 
        Uniswap: Permit2 & 58785 & 20571604 \\ \hline
    \end{tabular}
\end{table}


==> tables/2024_most_called_based_on_caller_number.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|}
    \hline
        to\_address & caller\_count & call\_count \\ \hline
        % 0x06450dee7fd2fb8e39061434babcfc05599a6fb8
        XEN crypto: XEN Token & 9442698 & 14431605 \\ \hline
        % 0xdac17f958d2ee523a2206206994597c13d831ec7 
        USDT & 8308677 & 82806179 \\ \hline
        % 0xa0b86991c6218b36c1d19d4a2e9eb0ce3606eb48 
        USDC & 3409866 & 54947812 \\ \hline
        % 0x0de8bf93da2f7eecb3d9169422413a9bef4ef628 
        CoinTool: XEN Batch Minter& 3114845 & 3422010 \\ \hline
        % 0x0a252663dbcc0b073063d6420a40319e438cfa59
        XEN Crypto: XENT Token& 3066096 & 5722312 \\ \hline
        % 0x3fc91a3afd70395cd496c647d5a6cc9d4b2b7fad 
        Uniswap: Universal Router & 2318539 & 42000820 \\ \hline
        % 0xc7ba94123464105a42f0f6c4093f0b16a5ce5c98 
        Unknown(deployed by Gitcoin Grantee)& 1651361 & 1809419 \\ \hline
        % 0xa9d1e08c7793af67e9d92fe308d5697fb81d3e43 
        CoinBase 10& 1148460 & 2703349 \\ \hline
        % 0xc02aaa39b223fe8d0a0e5c4f27ead9083c756cc2 
        WETH & 1089769 & 347585215 \\ \hline
        % 0x9a10da8ce77f26231860764a2caab36e70584c4b 
        AlphaPo: Hot 3& 880381 & 1031651 \\ \hline
    \end{tabular}
\end{table}

==> tables/all_call.tex <==


\begin{table*}[ht]
\centering
\begin{tabular}{|r|l|l|l|}
\hline
% \textbf{Callee Address} & 
\textbf{Count} & \textbf{Label} & \textbf{Proxy?} & \textbf{supplier}\\
\hline
% 0xc02aaa39b223fe8d0a0e5c4f27ead9083c756cc2 &
566,850,342 & Wrapped ETH & No & https://sky.money/\\
% 0xdac17f958d2ee523a2206206994597c13d831ec7 & 
293,795,251 & Tether Token & No & https://www.bitfinex.com/\\
% 0xa0b86991c6218b36c1d19d4a2e9eb0ce3606eb48 & 
125,159,306 & USDC Coin & Yes &Circlehttps://www.usdc.com/\\
% 0x7a250d5630b4cf539739df2c5dacb4c659f2488d https://www.coinbase.com/blog/usdc-v2-upgrading-a-multi-billion-dollar-erc-20-token& 
110,155,053 & Uniswap V2 Router & No &Uniswap \\
% 0x0000000000000000000000000000000000000001 & 
t66,760,962 & Pre-compile(0x01) & - &\\
% 0x3fc91a3afd70395cd496c647d5a6cc9d4b2b7fad & 
66,244,422 & Uniswap Universal Router & No & Uniswap\\
% 0xa5409ec958c83c3f309868babaca7c86dcb077c1 & 
62,045,415 & OpenSea Registry & No & Opensea\\
% 0x06450dee7fd2fb8e39061434babcfc05599a6fb8 & 
45,403,694 & XEN Token & No &https://xen.network/ \\
% 0x000000000022d473030f116ddee9f6b43ac78ba3 & 
38,838,029 & Uniswap Protocol: Permit2 & No &Uniswap\\
% 0xa3c1e324ca1ce40db73ed6026c4a177f099b5770 & 
33,864,039 & Bittrex: Controller & No &Bittrex Global(terminated) \\
\hline
\end{tabular}
\caption{Summary of Callee Addresses and Associated Counts}
\label{tab:callee_addresses_call}
\end{table*}

==> tables/all_delegatecall.tex <==

\begin{table*}[ht]
\centering
\begin{tabular}{|r|l|l|l|}
\hline
% \textbf{Callee Address} & 
\textbf{Count} & \textbf{Label} & \textbf{Proxy?} & \textbf{supplier}\\
\hline
% 0xa2327a938febf5fec13bacfb16ae10ecbc4cbdcf & delegatecall & 
109434644 & -FiatTokenV2\_1 & No & Circle\\
% 0x4bba9b6b49f3dfa6615f079e9d66b0aa68b04a4d & delegatecall 
87527375 & XEN Crypto & No & XEN\\
% 0x43506849d7c04f9138d1a2050bbf3a0c054402dd & delegatecall &  https://dashboard.tenderly.co/contract/mainnet/0x43506849d7c04f9138d1a2050bbf3a0c054402dd/transactions
54083426 & -FiatTokenV2\_2 & No & Circle?  \\
% 0x68b3465833fb72a70ecdf485e0e4c7bd8665fc45 & delegatecall & 
25764680 & Uniswap V3: Router 2 & Yes & Uniswap\\
% 0xb7277a6e95992041568d9391d09d0122023778a2 & delegatecall & 
21638736 & -FiatTokenV2 & No & Circle\\
% 0xf9e266af4bca5890e2781812cc6a6e89495a79f2 & delegatecall & 
21567513 & -AuthenticatedProxy & Yes & Opensea\\
% 0xd9db270c1b5e3bd161e8c8503c55ceabee709552 & delegatecall & 
14928768 & Safe: Singleton 1.3.0 & No & Gnosis \\
% 0x2b33cf282f867a7ff693a66e11b0fcc5552e4425 & delegatecall & 
12272397 & Lido: DAO Impl 1.0.0 & No & dev.izqui.eth\\ 
% 0xcca06cd29c61123d9d65b904b18174382380ca64 & delegatecall & 
12131916 & -Strong\_v2: ServiceV9
 & No & ?\\
% 0x0de8bf93da2f7eecb3d9169422413a9bef4ef628 & delegatecall & https://ct.app/batchMint/xen
11496529 & CoinTool: XEN Batch Minter & No & cointool\\
\hline
\end{tabular}
\caption{Summary of Callee Addresses(delegeatecall) }
\label{tab:callee_addresses_delegatecall}
\end{table*}

==> tables/all_staticcall.tex <==

\begin{table*}[ht]
\centering
\begin{tabular}{|r|l|l|l|}
\hline
% \textbf{Callee Address} & 
\textbf{Count} & \textbf{Label} & \textbf{Proxy?} & \textbf{supplier}\\
\hline
488425602 & Wrapped ETH & & \\
169122904 & 01 & - & - \\
109302905 & 02 & - & - \\
68418788 & USDC & Yes & Circle \\
53484668 & USDT & No & Bitfinex \\
42967120 & 06 & - & -\\
42884144 & 07 & - & -\\
22038903 & 04 & - & -\\
17785740 & DAI & No & Sky \\
16288458 & 05 & - & \\
\hline
\end{tabular}
\caption{Summary of Callee Addresses(delegeatecall) and Associated Counts}
\label{tab:callee_addresses_delegatecall}
\end{table*}

==> tables/calls_per_year.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|}
    \hline
        year & call\_traces\_count \\ \hline
        2015 & 1396570 \\ \hline
        2016 & 68533512 \\ \hline
        2017 & 153923782 \\ \hline
        2018 & 463680455 \\ \hline
        2019 & 552886859 \\ \hline
        2020 & 1078986855 \\ \hline
        2021 & 1637108480 \\ \hline
        2022 & 1659676996 \\ \hline
        2023 & 1929147230 \\ \hline
        2024 & 2396500599 \\ \hline
    \end{tabular}
\end{table}

==> tables/created_contracts_per_year.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|}
    \hline
        year & contract\_creations & distinct\_count \\ \hline
        2015 & 5724 & 5724 \\ \hline
        2016 & 213112 & 213112 \\ \hline
        2017 & 3726261 & 3726261 \\ \hline
        2018 & 5968989 & 5968989 \\ \hline
        2019 & 6314467 & 6314428 \\ \hline
        2020 & 16336491 & 16332172 \\ \hline
        2021 & 11150283 & 10994373 \\ \hline
        2022 & 7414824 & 7390280 \\ \hline
        2023 & 9052530 & 9050150 \\ \hline
        2024 & 3878047 & 3877467 \\ \hline
    \end{tabular}
\end{table}

==> tables/lido_transparency.tex <==
\begin{table*}
\centering
\begin{tabular}{|l|l|l|}
\hline
\textbf{Contract} & \textbf{Mainnet Ethereum Address} & \textbf{type} \\ \hline
Lido: DAO impl 1.0.0 & 0x2b33cf282f867a7ff693a66e11b0fcc5552e4425 & impl \\ \hline
stETH token Impl 2.0.0 & 0x17144556fd3424edc8fc8a4c940b2d04936d17eb & impl \\  \hline
Lido: Aragon Token Manager Impl &
0xde3A93028F2283cc28756B3674BD657eaFB992f4 & impl\\  \hline
Lido: Staking Router impl 1.0.0 &
0xd8784e748f59ba711fb5643191ec3fadd50fb6df & impl\\

\hline
\end{tabular}
\caption{Lido Transparency}
\label{tab:lido_trans}
\end{table*}


==> tables/subtraces.tex <==
% \usepackage{color}

\definecolor{Shark}{rgb}{0.113,0.113,0.125}
\begin{table}[h]
\centering
\caption{}
\label{tab:subtraces}
\begin{tblr}{
  cell{2}{2} = {fg=Shark},
  cell{3}{2} = {fg=Shark},
  cell{4}{2} = {fg=Shark},
  cell{5}{2} = {fg=Shark},
  vline{2} = {-}{},
  hline{2-5} = {-}{},
}
Subtraces  & \# Contracts \\
at least 0 & 11322760     \\
at least 1 & 11125379     \\
at least 2 & 10257161     \\
at least 3 & 704559       
\end{tblr}
\end{table}

==> tables/uniswap_v3.tex <==
\begin{table*}
\centering
\begin{tabular}{|l|l|}
\hline
\textbf{Contract} & \textbf{Mainnet Ethereum Address} \\ \hline
UniswapV3Factory & 0x1F98431c8aD98523631AE4a59f267346ea31F984 \\ \hline
Multicall & 0x1F98415757620B543A52E61c46B32eB19261F984 \\ \hline
Multicall2 & 0x5BA1e12693Dc8F9c48aAD8770482f4739bEeD696 \\ \hline
ProxyAdmin & 0xB753548F6E010e7e680BA186F9Ca1BdAB2E90cf2 \\ \hline
TickLens & 0xbfd8137f7d1516D3ea5cA83523914859ec47F573 \\ \hline
Quoter & 0xb27308f9F90D607463bb33eA1BeBb41C27CE5AB6 \\ \hline
SwapRouter & 0xE592427A0AEce92De3Edee1F18E0157C05861564 \\ \hline
NFTDescriptor & 0x42B24A95702b9986e82d421cC3568932790A48Ec \\ \hline
NonfungibleTokenPositionDescriptor & 0x91ae842A5Ffd8d12023116943e72A606179294f3 \\ \hline
TransparentUpgradeableProxy & 0xEe6A57eC80ea46401049E92587E52f5Ec1c24785 \\ \hline
NonfungiblePositionManager & 0xC36442b4a4522E871399CD717aBDD847Ab11FE88 \\ \hline
V3Migrator & 0xA5644E29708357803b5A882D272c41cC0dF92B34 \\ \hline
QuoterV2 & 0x61fFE014bA17989E743c5F6cB21bF9697530B21e \\ \hline
SwapRouter02 & 0x68b3465833fb72A70ecDF485E0e4C7bD8665Fc45 \\ \hline
Permit2 & 0x000000000022D473030F116dDEE9F6B43aC78BA3 \\ \hline
UniversalRouter & 0x3fC91A3afd70395Cd496C647d5a6CC9D4B2b7FAD \\ \hline
v3StakerAddress & 0xe34139463bA50bD61336E0c446Bd8C0867c6fE65 \\ \hline
\end{tabular}
\caption{Uniwap V3 Contract Addresses on Ethereum mainnet}
\label{tab:uniswapv3}
\end{table*}

